TraMNet - Transition Matrix Network for Efficient Action Tube Proposals

Current state-of-the-art methods solve spatiotemporal action localisation by extending 2D anchors to 3D-cuboid proposals on stacks of frames, to generate sets of temporally connected bounding boxes called \textit{action micro-tubes}. However, they fail to consider that the underlying anchor proposal hypotheses should also move (transition) from frame to frame, as the actor or the camera does. Assuming we evaluate $n$ 2D anchors in each frame, then the number of possible transitions from each 2D anchor to the next, for a sequence of $f$ consecutive frames, is in the order of $O(n^f)$, expensive even for small values of $f$. To avoid this problem, we introduce a Transition-Matrix-based Network (TraMNet) which relies on computing transition probabilities between anchor proposals while maximising their overlap with ground truth bounding boxes across frames, and enforcing sparsity via a transition threshold. As the resulting transition matrix is sparse and stochastic, this reduces the proposal hypothesis search space from $O(n^f)$ to the cardinality of the thresholded matrix. At training time, transitions are specific to cell locations of the feature maps, so that a sparse (efficient) transition matrix is used to train the network. At test time, a denser transition matrix can be obtained either by decreasing the threshold or by adding to it all the relative transitions originating from any cell location, allowing the network to handle transitions in the test data that might not have been present in the training data, and making detection translation-invariant. Finally, we show that our network can handle sparse annotations such as those available in the DALY dataset. We report extensive experiments on the DALY, UCF101-24 and Transformed-UCF101-24 datasets to support our claims.

==> text/approach.old.tex <==
\iffalse
\section{Methodology} \label{sec:methodology}
As outlined in Fig.~\ref{fig:algorithmOverview}, our approach takes two video frames that $\delta$ apart from one another, then they are fed through a base CNN which generates pyramid of feature maps at different level of depth in CNN network, in this case, we use SSD~\cite{liu15ssd} as base network (\S~\ref{subsec:base_net}-Fig.~\ref{fig:algorithmOverview}e).

The transition matrix is used to configure the pooling layers at each level of the pyramid. Pooled features are then supplied to two independent linear layers at each pyramid level to predict micro-tube and their scores. Each pooled feature is responsible to generate $2\times 4\times b$ boxes and $b$ score vectors of $C+1$ length for $C$ class and one for background class, where $b$ is number anchor boxes per grid location in feature map. 

\subsection{Base detection network} \label{subsec:intg_det_net}
Purpose of this work is to show the importance of using transition anchor boxes, which is applicable to untrimmed videos. Two state-of-the-art method from Singh \etal~\cite{singh2016online} and Kalogeiton \etal ~\cite{kalogeiton2017action} make use of SSD network with VGG~\cite{simonyan2014very} as base network. So, we choose SSD as base architecture. One can use 

Many other related works~\cite{he2017generic,hou2017tube,saha2017amtnet} make use of Faster-RCNN as base detection network, 
which is a two-stage pipeline and harder to train, but they can perform better than SSD, especially,
 on JHMDB21 dataset ~\cite{singh2016online} ~\cite{hou2017tube} in the context of action detection. 
 
 Recently, Lin \etal ~\cite{lin2017focal} has shown that single stage network can perform similarly to the two-stage networks using strong feature maps for source layers. 

 One can easily plug in more strong base representation networks, such as inflated 3D network by Carreira and Zisserman ~\cite{carreira2017quo}, 
 which is shown to work in action detection by Gu \etal ~\cite{ava2017gu}. 
 
 \fi
%  So, in the wake of new base detection networks reconfiguration of these networks using transition matrix would still be applicable and useful.  We will now focus on how transition matrix applied to select more overlapping prior anchor tubes with targeted tubes improves the spatiotemporal action localisation performance. 
%   %We believe this work would be applicable to finding object tubes in videos as well.
% 
% \subsection{Transition Matrix} \label{subsec:transition_matrix}
% We build the transition matrix using the ground truth boxes from consecutive frames that are $\delta$ apart. Grid cell location of frame anchor boxes or sometimes called prior regions~\cite{liu15ssd} will be called anchor regions.
% We want to find out how frequently max overlap with the target with one anchor region in the first frame moves to max overlap with another anchor region or itself in next frame.
% We can formulate this problem into an HMM, where each anchor regions $N$ anchor regions $A$ are fixed states and we want to learn how the sequence of ground truth boxes fit with probability. 
% 
% \textbf{HMM FORMULATION HER}
% 
% Our transition matrix is probabilistic in nature as we normalise each row of the matrix by the occurrence of ground truth in the first frame. This allows us to use same transition matrix for more frames. 
% 
% 
% \subsection{Convolution to Linear layer} 
% Original SSD~\cite{liu15ssd} used $3\times 3\times D$ convolutional kernels as head over feature maps in pyramid, where $D$ is the size of feature map. 
% Precisely, $4\times b$ kernels for bounding boxes prediction with $b$ aspect ratios of anchor boxes and $(C+1)\times b$ kernels for classification scores over each anchor region. Convolutional kernels are efficiently implemented in current deep learning libraries, however when we fix the number of kernels then that becomes the part of the fixed architecture of the network. In our case, we want to change the number of outputs depending upon the cordiality of transition matrix while keeping the number of parameters constant. To address that, we pool $3\times 3\times D$ features from each anchor region of feature map and stack them similarly pooled feature from the feature map of another frame. This will result in arbitrary number of pooled features of fixed dimension ($2\times 3\times 3\times D$), where number of features are decide based on transition matrix. 
% 
% 
% Now we can pass these features through a linear layer with $(12\times D) \times (4\times b)$ parameters for micro-tubes prediction layer and $(12\times D) \times (C+1)\times b)$ for classification layer, which is same as parameters used in convolutions kernels. 



% Another advantage of using linear layer is that we can use different transition matrix at evaluation time for e.g. we could fill all the diagonal elements missing in training data i.e. set the same anchor region to same anchor region to one which wasn't not present in training data. 

% \subsection{Appearance and flow cues} 
% Previous state-of-the-art works~\cite{kalogeiton2017action,singh2016online} on action localisation performs late fusion after detection boxes are produced by each individual network for appearance and optical low images. 
% For a fair comparison, we keep the trend and do late fusion from the outputs of appearance and flow networks. 
% Kalogeiton \etal ~\cite{kalogeiton2017action} showed that \textit{mean} fusion works better than \textit{boost} fusion ~\cite{Saha2016} or \textit{union-set} fusion~\cite{singh2016online}. Basically, fusion in done by taking the mean of the scores of each anchor predictions and micro-tube boxes from appearance stream are considered final micro-tube. We show all the results with mean fusion strategy, please refer to supplementary material for individual stream performance. 

% 
% \subsection{Detection network training and implementation.}
% We re-implemented SSD\cite{liu15ssd} network using pooling and linear heads rather than convolutional kernel and reproduced the results by Singh \etal~\cite{singh2016online}. Similarly, we reproduced the  works of Kalogeiton  \etal~\cite{kalogeiton2017action} using linear heads and cuboid of anchor tubes, in same spirit we re-implement AMTnet in with SSD as base network rather than Faster-RCNN in original work~\cite{saha2017amtnet}. We use consistent training setting for Kalogeiton \etal~\cite{kalogeiton2017action}, AMTnet~\cite{saha2017amtnet}, for e.g. while training on UCF101-24 dataset, we used  batch size of 16 and initial learning was set to $0.0005$ and learning rate drop after 100K iterations for appearance stream and 140K for flow stream, while appearance stream was only trained for 180K iteration flow stream was trained for 220K iterations. More details about the parameters and training setting is provided in supplementary material.

%and out proposed transition matrix network (TMnet), while transition for re-implemented version of SSD\cite{liu15ssd} %with linear layer (SSDL) are same as used by Singh \etal~\cite{singh2016online}, where  In cases of networks, batch %size was set to 16 and initial learning set to $0.0005$ and learning rate drop after 100K iterations for appearance %stream and 
%We use a learning rate of $0.0005$ for both the streams, 
%whereas that for JHMDB is set to $0.0001$ for both appearance and flow. 
%More implementation details are in the supplementary material.

\subsection{Online Tube Generation and temporal trimming}\label{subsub:algo}
We use online tube generation method proposed by ~\cite{singh2016online} with some modification, it is based on simple online tracking hypothesis. While Singh \etal ~\cite{singh2016online} conect frame-level detection across time we modify it to contact micro-tubes, where end of one micro-tube is connected to start of another. Similar to ~\cite{singh2016online}, we build action tracks incrementally by contacting micro-tubes across time, in out case, end of one micro-tube falls same frame where start of another micro-tube. If we have two micro-tubes, one from frame 1 to 6 and and another one from frame 6 to 11 then these tubes can be connected at frame 6. 
Kalogeiton \etal~ \cite{kalogeiton2017action} also adapts the linking process proposed by Singh \etal~\cite{singh2016online} to link tubelets. We handle temporal trimming labelling problem using dynamic programming  ~\cite{Saha2016,Evangel-2014}. We will show that temporal trimming aspect doesn't help in UCF101-24, in-fact it hurts the performance, but it helps in DALY dataset which has only only 4\% of the video duration is covered by action instances.


==> text/rebuttal_text.tex <==
%\vspace{-3mm}
\textbf{Intro} We thank the reviewers for appreciating the need of anchor micro-tubes. 
We would like to highlight three main points overlooked.
Firstly, our method is applicable to sparse annotations in principle way, e.g. AVA and DALY, unlike ACT-L or AMTNet-L which simply extend anchor cuboids.
Secondly, the evaluation of all possible anchor micro-tubes is intractable from training and GPU memory perspectives.
Thirdly, at test time we could use more generic anchor micro-tubes (L583-L590). %, which is the reason we focus in utilising the training data efficiently while maintaining speed and improving accuracy of AMTNet. 

\textbf{Reviewer 1: } 
%he HMM formulation seems problematic: it learns to predict transition matrix from a feature map location (x_t, y_t) to another (x_{t+1}, y_{t+1}), which is not translation invariant, as a result, same action at different locations may have very different anchors generated. Besides, the state is based purely on locations but not on visual appearances, and the sampling is deterministic, as a result, the generated anchors cannot handle different motion patterns.
\textit{\textbf{A}. The HMM formulation seems problematic: translation invariant. not based on visual appearances, and the sampling is deterministic. }
\textbf{Ans}: \textbf{\textit{Appearance:}} Anchor micro-tubes are generated based on the ground truth(GT), 
GT is generated by human annotators based on appearance and network learn to 
verify anchor micro-tubes based on appearance and motion both at train time and used to verify them at test time.
As oppose to tracking anchors based on appearance [29] we think that anchor micro-tube is better solution, 
especially when annotations are spares (DALY or AVA) i.e. train $\Delta$ is high and directly provide linked detections (i.e. micro-tubes).% for two frames.  
\textbf{\textit{Translation invariance:}} at test time, it can be handled by incorporating more anchor micro-tubes.
%We need fixed set of hypotheses as noted by the reviewer 3 to measure IoU between ground truth and anchor micro-tubes to compute loss. 
Traditionally anchors are user defined for each frame in object detectors like prior boxes in SSD or anchor boxes in RPN of faster RCNN. 
If we are to define all possible anchor micro-tubes for SSD-300 it would 76+($r^2$ ($r$=8732)) million
%and trillions anchor micro-tubes in latest detector FPN or RetinaNet 
for just 2 frames, which is intractable from training and GPU memory perspectives. 
We noticed that we could utilise the anchor micro-tube's distribution from the training set to handle training process efficiently.
At test time, we could have lot more anchor mirco-tubes (which are translation invariant) 
to cover the variation in test set once the classification and regression heads are trained, 
given that the network's evaluation step is much faster and memory efficient. 
To rebut, we have evaluated using all possible combinations with neighbours cells to generate anchor micro-tubes 
(i.e. training transition matrix (TM) + diagonal of TM + translations to 8 neighbouring cells) at test time, 
similar to experiment described in L583-L590 we observed no performance difference.
The reason may be due to the fact that in UCF-101-24 the variance in translation of anchor boxes is nearly same for both train and test sets.
\textbf{\textit{Sampling}} is not deterministic as it relies on the distribution of training data. It is sampled based on transition probability threshold, 
which results in varying number of anchor micro-tubes, one can sample fixed the number of top anchor micro-tubes using MCMC sampling based on the transition probability. 
But this is equivalent to varying the threshold. Please see the ablation study on the effects of transition threshold in point D.
% it is may be because translation distribution of actors in UCF101-24 dataset is same during training and test time. 
% More importantly, it strengthens our point that we can train classification and regression heads using transition matrix and have more anchors at test time without sacrificing training performance. 


%HMM requires groundtruth to train, which may not be necessarily available (for example, for AVA the groundtruth annotations are 1-second apart)
\textit{\textbf{B}. HMM requires GT to train, not necessarily available (e.g. AVA, GT annotations are 1-second apart }
\textbf{Ans}: This is why we focus handling sparse annotation in DALY dataset. 
Approaches like ACT-L requires to have ground truth of consecutive frames. 
Whereas, our model utilises ground truth data that is $\Delta$ frames apart, e.g., 
1 seconds in AVA, 2.3 seconds on an average in DALY.
At the test time, this $\Delta$ could be reduced to have dense predictions, 
which we found to be more helpful as shown in Table 1 and 2 that 
test $\Delta$ is independent of train $\Delta$ and discussed in section 4.3.

%- The presentation could be improved, it is a bit difficult to follow Figure 2 and 3 without referring to the text.
\textit{\textbf{C}. The presentation could be improved. }
\textbf{Ans}: We will work on it to improve. 

%- The experiments could be improved. The paper compares with other state-of-the-art methods but lacks ablation experiments of the proposed method, how are different design choices affect the learned anchors? It's also important to visualize the learned anchors.
\textit{\textbf{D}. The experiments could be improved... Visualise the learned anchors... }
\textbf{Ans}: For visualisation we provide heat maps of transition matrices, 
which indicate how off diagonal elements appear more as the training $\Delta$
increase which highlights the need of anchor micro-tubes over anchor cuboids,
especially when annotations are sparse (AVA or DALY).
\textit{Ablation studies} (1). We tried different train and test $\Delta$s as shown in table 1 and discussed in section 4.3.
(2) We cross-validated different transition thresholds on transition matrix. As asked by reviewer 2, transition threshold on transition probability of $2\%$ $5\%$ $10\%$ $15\%$ and $20\%$ produces the Avg-video-mAP of $21.6\%$ $22.0\%$ $22.4\%$ $21.9\%$ $21.2\%$ on appearance stream. (3) Class-wise results in supplementary material.
(4) \textbf{please specify the experiments we should conduct for future submission?}

%The proposed method is ad-hoc. The transition matrix is estimated separately from the network and a hard threshold is used. Instead, a fully end-to-end model is preferred. For example, ideas like spatial transformer network may be used to estimate the spatial transformation between two frames. 
\textbf{Reviewer 2: } \textit{A. Method is ad-hoc. TM is estimated separately. why not a fully end-to-end model? }
\textbf{Ans}: A fully end-to-end model would require to evaluate all 76+m anchors (see answer to reviewer 1's point A), 
consequently, which leads to intractability and GPU memory limitations. Which is why AMTNet and ACT used anchor cuboids.
%Our approach learns which anchor to use at training time by exploiting the HMM's transition properties in principle way.
%Linear heads needs to be trained to regress the offsets from anchor micro-tubes,
%where anchor micro-tubes with IoU more than 0.5 with ground truth, So, 
%why not use it to boost the efficiency of training while still maintaining 
%the gains from anchor micro-tubes rather over anchor cuboids.  

%Since the major contribution comes from the transition matrix, more experiments around the transition matrix may be interesting. For example, how about using different thresholds, what are the impact off-diagonal entries?
\textit{\textbf{B}. more experiments for thresholds... }
\textbf{Ans}: See answer to reviewer 1's point D. 

%c. The experimental results are not very impressive. On UCF101, for several classes highlighted (classes with spatial movement) in supplementary materials, the proposed method performs worse (IceDancing, LongJump, Pole Vault, FloorGymnastics), it may be interesting to look into the reason.
\textit{\textbf{C}. Results are not very impressive... }
\textbf{Ans}: Our method performs better than the baseline AMTNet-L (uses 2 frames) on
both UCF101 and DALY dataset and very much similar to 6 frame method ACT-L. 
Our method works on spares annotations of DALY, 
whereas ACT-L are not applicable
and AMTnet performs much worse than ours.

%- The main novelty of the paper is the introduction of "anchor micro-tube". It is necessary to evaluate these anchors, in terms of number of anchors, IoU with ground-truth, etc. As far as I have understood, baselines are: cuboids as in ACT-L [11], pairs of anchor boxes as in AMTnet-L [10]. Video-mAP reported in Table 1 include too many postprocessing stages (linking micro tubes + trimming) which make harder a comparison between the resulting output of the network. Maybe frame-mAP [11] would be more relevant for that ; and would allow to report mAP according to the speed of the actor.
\textbf{Reviewer 3. }
\textit{\textbf{A}. Baselines comparison with ACT-L [11] and AMTnet-L [10] (linking micro tubes + trimming could hamper). Why not frame-mAP [11]? }
\textbf{Ans}: To make fair comparison, we re-implemented [10] and [11] with linear layers and used excatly the same post-processing steps for [10], [11] and ours (TraMNet). Only difference in AMTnet-L, ACT-L and TraMNet is the kind of anchors are used. We also used the same set of hyper-parameters noted in L475-485. We are trying to improve linking process which is reflected in video-mAP rather than frame-mAP. Frame-mAP for AMTNet-L, ACT-L and TraMNet-L is $63.2$ $62.8$ and $63.5$ respectively, whereas avg-video-mAP is $21.6$ $22.4$ and $22.4$ respectively on appearance stream. 

%- In a more general perspective, I would imagine that anchor micro tubes should be specific to the few frames that are seen, ie, depend on the content. 
% I mean, the proposed approach learns from the micro-tube shape of the training set alone. 
% By definition, one would like the anchor micro-tubes to "follow"/"cover" a similar content/object/actor across time, 
% thus this content should be kind of "tracked". 
% The proposed approach only relies on box coordinates and is likely to contain a lot of irrelevant proposals for each video, 
% and maybe to miss some obvious in case of unseen shape of micro-tubes at test time. 
% This is probably why the authors limit the micro-tubes to two frames. This is a clear advantage of [29] compared to the proposed approach.
\textit{\textbf{B}. Why not tracked [29] and unseen micro-tubes at test time. }
\textbf{Ans}: For both points please refer to the answer to the point A of reviewer 1.
% - The proposed approach basically learn micro-tubes from the training tubes. Actually, doing a k-means [15] on the micro-tubes from training set should be another baseline in the evaluation.
\textit{\textbf{C}. k-means [15] on the micro-tubes should be another baseline. }
\textbf{Ans}: %Yes, it is possible to do it, but 
k-means in [15] is applied to find out 
aspect ratios and scales of anchor boxes on all grid locations. 
Which applicable to any detection method AMTnet, ACT, any other or ours, we wanted to see 
how transition across cell can be handled and keep the comparison with AMTNet and ACT fair.  

% - In a similar spirit, I would imagine that anchor micro tubes are not dependent on the x,y coordinates. 
% I mean, the transition matrix can be also learn with a relative cell offset instead of an absolute cell position. 
% This would have the advantage of being translation-invariant.

\textit{\textbf{D}. Translation-invariant }
\textbf{Ans}: please answer to reviewer 1's point A.

% - The method cannot contain anchors micro-tubes coming from different scales, ie, may fail in case of change of distance between the camera and the distance. Also, it assumes that the anchor of index rho in [0...r] in a cell match with the same index rho in another cell, which clearly limits the set of possibilities. One way to avoid that might actually be to consider $r^2$ anchor inside each pair of cells.

\textit{\textbf{E}. micro-tubes from different scales.. } \textbf{Ans}: We acknowledged it in L344-L347.% For, now we leave it for future work.

% - The part on the "reconfigurable pooling layer" makes think that this is novel, but there is nothing new in the pooling. The only thing is that between two sets of experiments, the number of proposals vary, but is fixed inside a given training / test. So it not really "reconfigurable". Actually, the use of "varies with time" in L368 is extremely misleading. It sounds like it changes with the time of a given video. As far as I have understood, this is just varying between two different experimentations with two different transition matrices.

\textit{\textbf{F}. ``reconfigurable pooling layer'' is nothing new}
\textbf{Ans}: One could say that this is just a re-implementation of convolution layer in linear layer, 
but this allows us to use different transition matrix at train and test test. 
We don't mean to mislead in L368, we will correct it. ``reconfigurable'' 
 mean that we could use different transition matrix at train and test time, % thanks to our pooling layer. 
%Hence able to train efficiently and test lot more anchor micro-tubes at test time 
hence, allows to cover variation in train and test time. % as mentioned in the answer to reviewer 1's point A. 

We will address the minor issues in the final version of the paper. 


==> text/supp_details.tex <==
In this supplementary material, we first present implementation details in Section~\ref{subsec:details}.
Next, we show how optical flow and appearance based feature contribute to the final performance 
in Section~\ref{sec:Contribution}.
Finally, we show how the transition matrix helps in dynamic classes over AMTNet-L in Section~\ref{sec:classes}.


\section{Implementation details}\label{subsec:details}

All models are trained with a batch size of $16$ on two 1080Ti GPUs (11GB VRAM each) for AMTNet-L and TraMNet.
Whereas, ACT-L is trained on 4 GPUs because it requires fitting feature maps of 6 frame into GPU memory.
We used Pytorch library to implement all the models (ACT-L, AMTnet-L, and TraMNet) by following the implementation of Singh \etal \cite{singh2016online} closely from their
% \url{ GitHub repository}{https://github.com/gurkirt/realtime-action-detection}.
\href{https://github.com/gurkirt/realtime-action-detection}{GitHub repository}.

\textbf{UCF1101-24.} We trained all our models using the data-loader function provided by Singh \etal~\cite{singh2016online} where 5000 training images are picked for each class to train.
The RGB stream is trained with an initial learning rate of $0.001$ and it is dropped by a factor of $10$ after $110K$ iterations, and the model is trained for $180K$ iterations for all the different detection frameworks, i.e., ACT-L, AMTMet-L, and TraMNet.
The flow stream is trained with an initial learning rate of $0.001$ and it is dropped by a factor of $10$ after $150K$ iterations, and the model is trained for $220K$ iterations for all the different detection frameworks, i.e., ACT-L, AMTMet-L, and TraMNet.


\textbf{DALY.} We use all the action instances of actions available even if 
the number of frames annotated in a given instance is less than 2. AMTNet-L and 
TraMNet requires at least two consecutive frames to train, but in case of 
DALY dataset, there are action instances where only one frame is annotated, we use annotated 
frame twice to make a sequence of two frames, as mentioned in the paper 
this happens for $12\%$ of action instances.
Remaining instances contribute according to the number of frames annotated per instance.

The RGB stream is trained with an initial learning rate of $0.001$ and it is dropped by a factor of $10$ after $12K$ iterations, and the model is trained for $30K$ iterations for all the different detection frameworks, i.e., AMTNet-L and TraMNet.
The Flow stream is trained with an initial learning rate of $0.001$ and it is dropped by a factor of $10$ after $15K$ iterations, and the model is trained for $50K$ iterations for all the different detection frameworks, i.e., AMTNet-L and TraMNet.

\textbf{Input Data Preparations.}
The number of input video frames to CNNs is more than $1$ in our case, e.g., $6$ for ACT-L action detection framework. 
The optical flow stream uses a stack of 5 frames as input for each input training example in the sequence.
In our case, sequence length ($s$) is more than (in case AMTNet-L and TraMNet equal to 2 and ACT-L equal to 6), 
so 2 or 6 ($s=2$) stacks of 5 frames are used as input for flow stream in case of TraMNet for flow stream.


The number of input frames for the RGB stream is equal to the sequence length, e.g., 2 for TraMNet.
Each optical flow image is a 3 channel image, where first two channels are flow in  $x$ and $y$ direction respectively and the third channel is the magnitude (square-root of the sum of squares) of flow in both directions.
We computed dense optical flow between each pair of successive video frames using the algorithms of~\cite{Brox-2004}.

The SSD relies on \textbf{data augmentation} to boost the performance, we extended the data augmentation~\cite{liu15ssd} function provided by Singh \etal \cite{singh2016online} in  their
\href{https://github.com/gurkirt/realtime-action-detection}{GitHub repository} to pass as input a sequence of frames in place of a single frame.
The same data augmentation was applied to all the frames in a training batch.

\textbf{VGG weight initialisation.}
The weights of VGG network (base network) are initialised with weights from a pre-trained ImageNet model~\cite{liu2015parsenet}\footnote{\url{https://gist.github.com/weiliu89/2ed6e13bfd5b57cf81d6}}
for appearance- and flow-based SSD networks for both UCF101-24 and DALY dataset.


\section{RGB and Flow Contribution}\label{sec:Contribution}
In Figure~\ref{table:ucf101_contrib}, we show how each stream individually performs and contributes the performance of fused model using \textit{mean-fusion}~\cite{kalogeiton2017action}.
We can observe that the RGB stream works better than the flow stream and fusion always gives improvements over the RGB stream.
Interestingly, the RGB stream is most dominant and performs comparable to the fusion model, hence one can only use RGB stream to improve the run-time speed of the whole system at the cost of a small performance drop.

\begin{table}[t]
  %\vskip -3mm
  \centering
  \setlength{\tabcolsep}{3.5pt}
  \caption{Action localisation results on untrimmed videos from UCF101-24 split1.
  The table is divided into 4 parts. The first part lists approaches which have single frames as input;
  the second part approaches which take multiple frames as input;
  the third part contemplates the reimplemented versions of approaches in the second group;
  lastly, we report TraMNet's performance.}
  \vskip 1mm
  {\footnotesize
  \scalebox{1}{
  \begin{tabular}{lccccccc}
  \toprule
  Methods & Train $\Delta$ & Test $\Delta$	&$\delta$ = 0.2   &$\delta$ = 0.5 & $\delta$ = 0.75 & $\delta$ = .5:.95 & Acc \% \\ \midrule
  %Yu \etal~\cite{yu2015fast} &NA &NA & 26.5  & --   & -- & -- & --\\
  %Weinzaepfel ~\cite{Weinzaepfel-2015}  & NA &NA & 46.8  & --   & -- & -- & --\\
  T-CNN~\cite{hou2017tube} & NA &NA & 47.1  & --   & -- & -- & --\\
  MR-TS~\cite{peng2016eccv}	 & NA &NA & 73.5  & 32.1 & 02.7 & 07.3 & --\\
  Saha~\etal~\cite{Saha2016}    & NA &NA & 66.6  & 36.4 & 07.9 & 14.4 & --\\
  SSD~\cite{singh2016online}    & NA & NA & 73.2 & 46.3 & 15.0 & 20.4 & --\\\midrule
  AMTnet~\cite{saha2017amtnet} rgb-only  & 1,2,3 & 1 & 63.0  & 33.1 & 00.5 & 10.7 & --\\
  ACT~\cite{kalogeiton2017action}   & 1 & 1 & 76.2  & 49.2 & 19.7 & 23.4 & --\\
  Gu \etal~\cite{ava2017gu} (\cite{peng2016eccv} + \cite{carreira2017quo})   & NA & NA & --  & \textbf{59.9} & -- & -- & --\\
  \midrule
  SSD-L with-trimming  & NA & NA & 76.2 & 45.5 & 16.4 & 20.6  & 92.0 \\
  SSD-L     & NA & NA & 76.8 & 48.2 & 17.0 & 21.7  & 92.1 \\
  ACT-L RGB               & 1 & 1 & 74.2 & 47.9 & 18.6 & 22.4  & 88.0 \\
  ACT-L Flow              & 1 & 1 & 72.8 & 43.9 & 12.3 & 18.6  & 86.2 \\
  ACT-L RGB+Flow          & 1 & 1 & 77.9 & 50.8 & 19.8 & \textbf{23.9}  & 91.4 \\
  AMTnet-L RGB            & 1 & 1 & 76.2 & 46.9 & 18.0 & 21.9  & 89.1 \\
  AMTnet-L Flow           & 1 & 1 & 73.7 & 43.6 & 11.3 & 17.5  & 88.2 \\
  AMTnet-L RGB+Flow       & 1 & 1 & \textbf{79.4} & \textbf{51.2} & 19.0 & 23.4  & \textbf{92.9} \\ \midrule
  TraMNet (ours) RGB      & 1 & 1 & 76.8 & 46.9 & 18.9 & 22.2  & 88.5 \\
  TraMNet (ours) Flow     & 1 & 1 & 74.9 & 43.1 & 11.2 & 17.6  & 87.1 \\
  TraMNet (ours) RGB+FLow & 1 & 1 & 79.0 & 50.9 & \textbf{20.1} & \textbf{23.9}  & 92.4 \\\bottomrule
  \end{tabular}
  }
  }
  %\vspace*{-\baselineskip}
  \label{table:ucf101_contrib} \vspace{-5mm}
\end{table}


\section{Ablation Study: Performance on Classes with Movements}\label{sec:classes}
There are many action classes with a lot of spatial movement in the UCF101-24 dataset, unlike DALY dataset where only ``CleaningFloor'' had spatial movements.
In Table \ref{table:ablation-study-ucf10102}, we show class-wise performance at detection threshold $\delta=0.2$.
We consider a class to have a considerable spatial movements if the class contributes to the off-diagonal elements in the transition matrix at $\Delta = 5$.
The ``BasketballDunk'', ``Skiing'', ``VolleyballSpiking'' are the classes which contribute most to the off-diagonal entries in the transition matrix.
It is clear from the Table \ref{table:ablation-study-ucf10102} that the transition matrix helps to improve the detection performance considerably for those classes (highlighted in red) which have signifiacnt spatial movements.
It is important to note that we build a transition matrix for each scale separately, our method is limited in case of when an actor moves towards or away from camera, or camera moves in that direction.
One such case is biking observed from the front view of the biker.
Solution to cover such movements is to build one transition matrix for all the pyramids.
However, our base network is SSD, which has inconsistent feature dimension across the scales of the pyramid, hence, concatenated features from different scales would result in inconsistent dimensionality.

The classes with multiple actors (e.g. ``IceDancing'', ``SalsaSpin'', ``Fencing'') suffer in the TraMNet framework.
We think it is due to the fact that the anchor micro-tubes are 
class invariant and movement of some classes might be creating confusion in these classes.
Adding class-specific anchor micro-tubes and respectively 
making regression layers class specific could help alleviate this problem.
In some static classes (e.g. ``GlofSwing'' or ``TennisSwing'')
we observe that TraMNet is better than both ACT-L and AMTNet-L, 
where as in other static classes (e.g. ``CricketBowling'' and ``RopeClimbing''), ACT-L is better.
We think it because ACT uses features from 6 frames and able to classify the classes better.


\begin{table*}
\vspace{5mm}
\centering
\footnotesize
\caption{Spatio-temporal detection results (video APs in $\%$) on UCF101-24 at $\delta=0.2$. Classes with movement in the dataset are highlighted in red colour.  }
\scalebox{0.60}{
\begin{tabular}{lcccccccc}
\toprule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Actions		     		& Basketball  &   \red{BasketballDunk} &   Biking &   \red{CliffDiving} &   CricketBowling &   \red{Diving} &   Fencing & \red{FloorGymnastics}  \\ \midrule
ACT-L & 50.3 & 78.0 & 78.3 & 79.2 & 70.5 & 100.0 & 89.9 & 98.9 \\
AMTNet-L & 53.6 & 79.4 & 82.2 & 81.7 & 65.7 & 100.0 & 90.7 & 99.5 \\
TraMNet & 51.9 & 81.8 & 80.0 & 81.6 & 60.6 & 100.0 & 87.0 & 98.8 \\ \midrule \midrule
Actions 			& GolfSwing   &   HorseRiding & IceDancing &   \red{LongJump} & PoleVault &   RopeClimbing &   SalsaSpin &  SkateBoarding \\ \midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
ACT-L & 69.8 & 96.1 & 87.9 & 81.9 & 88.9 & 99.4 & 43.6 & 89.8 \\
AMTNet-L & 77.6 & 96.1 & 86.5 & 88.6 & 92.9 & 98.1 & 46.9 & 88.0 \\
TraMNet & 76.5 & 96.1 & 83.5 & 86.6 & 88.8 & 97.7 & 41.7 & 89.2 \\  \midrule \\ \midrule
Actions  &   \red{Skiing} & \red{Skijet} & SoccerJuggling & Surfing & TennisSwing & TrampolineJumping & \red{VolleyballSpiking} & WalkingWithDog  \\ \midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
ACT-L & 81.1 & 87.8 & 95.0 & 67.0 & 35.0 & 67.6 & 44.0 & 90.4 \\
AMTNet-L & 82.4 & 93.5 & 94.9 & 68.9 & 40.5 & 65.7 & 42.0 & 90.4 \\
TraMNet & 85.2 & 93.6 & 94.4 & 65.6 & 42.8 & 66.8 & 53.5 & 91.2 \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\label{table:ablation-study-ucf10102}
\end{table*}

